Geometry Depth Consistency in RGBD Relative Pose Estimation

Relative pose estimation for RGBD cameras is crucial in a number of applications. Previous approaches either rely on the RGB aspect of the images to estimate pose thus not fully making use of depth in the estimation process or estimate pose from the 3D cloud of points that each image produces, thus not making full use of RGB information. This paper shows that if one pair of correspondences is hypothesized from the RGB-based ranked-ordered correspondence list, then the space of remaining correspondences is restricted to corresponding pairs of curves nested around the hypothesized correspondence, implicitly capturing depth consistency. This simple Geometric Depth Constraint (GDC) significantly reduces potential matches. In effect this becomes a filter on possible correspondences that helps reduce the number of outliers and thus expedites RANSAC significantly. As such, the same budget of time allows for more RANSAC iterations and therefore additional robustness and a significant speedup. In addition, the paper proposed a Nested RANSAC approach that also speeds up the process, as shown through experiments on TUM, ICL-NUIM, and RGBD Scenes v2 datasets.

==> sec/2_RelatedWorks.tex <==
\section{Related Works}

RGBD camera has been widely used in various VO~\cite{christensen2019edge, yuan2021rgb, zhao2023edgevo, ZHAO2023112487, yang2023resource} or SLAM~\cite{mur2017orb, schops2019bad, fontan2023sid, zhu2022nice} algorithms. It enables estimating a camera pose from three point correspondences which is typically processed under a RANSAC scheme. In conjunction with RGBD generated 3D point clouds,~\cite{li20232d3d} aimed to train a promising detector-free feature matching network based on 2D and 3D features. Though 80


% Even though modern learned detector-free matching approaches~\cite{sarlin2020superglue, sun2021loftr} mitigates such situations by constructing accurate dense correspondences before the RANSAC loop starts,


